Accelerating Parameter Extraction of Power MOSFET Models Using Automatic Differentiation

The extraction of the model parameters is as important as the development of compact model itself because simulation accuracy is fully determined by the accuracy of the parameters used. This study proposes an efficient model-parameter extraction method for compact models of power MOSFETs. The proposed method employs automatic differentiation (AD), which is extensively used for training artificial neural networks. In the proposed AD-based parameter extraction, gradient of all the model parameters is analytically calculated by forming a graph that facilitates the backward propagation of errors. Based on the calculated gradient, computationally intensive numerical differentiation is eliminated and the model parameters are efficiently optimized. Experiments are conducted to fit current and capacitance characteristics of commercially available silicon carbide MOSFET using power MOSFET models having 13 model parameters. Results demonstrated that the proposed method could successfully derive the model parameters 3.50x faster than a conventional numerical-differentiation method while achieving the equal accuracy.

==> tex/append.tex <==
{\sntn{
\section*{Appendix}
The proposed method can be applied {\sato{even}} when the model contains loops, such
as ``while'' or ``for'' statements. The computational graph of the
loop is constructed with a feedback loop.  In the forward mode, the
computational graph is repeatedly traversed until the convergence
condition is satisfied.  Here, the variables of the graph are extended
to use a {\it stack} data structure so that the intermediate values
for each calculation are pushed into it. The backward mode is
conducted by popping the variables while traversing the graph. Here,
the while statement essentially contains a conditional branch.
Meanwhile, some models also contain ``if'' statement, so that
different calculations are carried out depending on the bias condition
or the parameter. In the proposed method, the conditional branch is
realized by adding a flag to the node again as a stack to judge which
path should be selected. The backward mode is carried out by
traversing the graph according to the flag value.
}}

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.65\linewidth]{./loop.pdf}
  \caption{{\sntn{Example of a computational graph for a while loop.}}}
  \label{fig:loop}
\end{figure}

{\sntn{
Fig.~\ref{fig:loop} shows a computational graph of a while statement
in the following code snippet as an example.}}
\begin{lstlisting}[basicstyle=\ttfamily]
  val = 10;
  while (val > 0.5){
    val = val / 2;
  }
\end{lstlisting}
{\sntn{
In this code, variable {\tt val} is initialized to 10, then changes to
5, 2.5, 1.25, 0.625, and 0.3125.  Finally, the loop terminates when
its value becomes smaller than 0.5.  The computational graph of the
while statement is constructed with a feedback loop containing a
conditional branch and stacks as shown in Fig.~\ref{fig:loop}. In the
forward mode, the model equation is evaluated while pushing the value
of variable {\tt val} into the stack sequentially.  In addition,
%stack
the flags that will be used to which path should be evaluated
are stored in the stack.  Then, in the backward mode, the graph is
traversed by popping these values.
}}


==> tex/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

Herein, we proposed a novel parameter-extraction method that is applicable
to various power MOSFET models. The proposed method employs AD, which is
commonly used in backpropagation of artificial neural networks. The AD
technique involves the calculation of the partial derivatives according to
the chain rule by simply traversing the calculation graph, thereby reducing
the number of times the model equation must be evaluated compared to ND
calculation. Due to this improvement, the AD approach requires less
computation time than the ND approach for parameter extraction. Experimental
results using a commercial SiC power MOSFET demonstrated that the proposed
method could be used to successfully derive the model parameters for the
current equation of the MOSFET about 4.3 times faster than the conventional
gradient-descent method using two-point gradient approximations.

% {\mmm{In future studies, to show the effectiveness of the proposed
% method in practice, the applicability of a combinational usage of the
% proposed method and other optimization algorithms needs to be investigated. For
% example, the proposed method can be incorporated into the LM-based
% parameter extraction {\sato{that uses Jacobian in the optimization,
% which}} is widely {\sato{utilized}} in the industrial device modeling
% flow~\cite{iccap}.

% introducing the combination, further improvement is expected since the
%calculation time of derivatives and the iteration number are reduced.
In future study, we intend to include an evaluation with open source
packages for AD as introduced in~\cite{autodiff} to analyze more
complex descriptions in arbitrary power MOSFET models by the
computational graph. {\sntn{In addition, the evaluation of the proposed
method is still limited in the static characteristics. We intend to
investigate a further evaluation on the dynamic characteristics based
on the extracted parameters.}}


% {\shintani{
% Our future work includes to investigate an applicability of a
% forward-type-AD-based parameter extraction. As presented in
% Section~\ref{sec:multi} the effectiveness of the parameter extraction is not
% so high for the model with few model parameters, such as $\cds$ and
% $\cgd$. Hence, further accerelation could be achieve by the combinational
% usage of the forward-type AD and reverce-type AD.}}



==> tex/conv.tex <==
\section{Parameter extraction based on numerical differentiation}
\label{sec:conv}

\subsection{Gradient-Based Parameter Extraction}
We first review gradient-based parameter extraction as the typical
optimization algorithm, while the proposed method is applicable to
other algorithms using derivatives, such as the Levenberg-Marquardt
(LM) method~\cite{SIAM1963_Marquardt}.  Algorithm~\ref{alg:gd}
outlines the parameter extraction for a drain current model,
$f(\cdot)$, as an example. Here, $f(\cdot)$ is a function of the
gate-source voltage, $V_{\rm gs}$, and drain-source voltage, $V_{\rm
  ds}$, and is based on the current model equation with constant model
parameters, $\bm p$.

The algorithm has the following seven inputs: the initial value vector of
the model parameters ($\bm p$), the vector representing the small changes in
each parameter ($\bm{\delta}$), the measured current data
($\bm{I}^{\rm meas}$) and the corresponding bias voltages ($\bm{V}$), the
target error ($E_{\rm target}$), and the maximum number of iterations
($N_{\rm max}$). $\bm{\eta}$ represents the rate at which the parameters are
updated. Vectors $\bm{p}$, $\bm{\delta}$, and $\bm{\eta}$ all have sizes of
$n$, which is equal to the number of model parameters. $\bm{V}$ is a vector
whose components represent the voltage pair $V_{\rm gs}$ and ${V_{\rm ds}}$
at which the drain current, $\bm{I}^{\rm meas}$, is measured. Vectors
$\bm{V}$ and $\bm{I}^{\rm meas}$ both have dimensions of
$m_{\rm vd} \times m_{\rm vg}$, where $m = m_{\rm vd} \times m_{\rm vg}$ is
the total number of the data points measured and $m_{\rm vd}$ and
$m_{\rm vg}$ are the number of voltages measured in the ${V_{\rm ds}}$ and
${V_{\rm gs}}$ sweeps, respectively.

The gradient-based parameter extraction proceeds by changing each of the
parameters, $\bm{p}$, in the direction determined by the numerical
derivatives to reduce the cost function, $E$. Here, $E$ is the
root-mean-square error (RMSE) between the simulation and measurement and is
generally defined as follows:
\begin{equation}
  E = \sqrt{\frac{1}{m}\sum_{j=0}^{m-1} (I^{\rm meas}_j-I^{\rm sim}_j)^2}.
  \label{eq:error}
\end{equation}
Before the extraction is initiated, the currents may be normalized such
that each bias point has an equal contribution to the final
error~\cite{TED2008_Takeuchi}.  Otherwise, the fitting results would be
dominated by the bias points having larger current values, while those
having smaller current values do not contribute to the fitting.  This
leads to insufficient extraction accuracy.
%{\shintani{In {\sato{practice}}, the residual of conductance normalized
%by early voltage {\sato{may}} also {\sato{be}} used {\sato{replacing}}
%the current {\sato{error metric}} in Eq.~(\ref{eq:error}).}}
%% {\sato{Other error metrics can also be used in place of or in addition
%%     to~(\ref{eq:error}) {\mmm{as presented in~\cite{TED1997_Cheng}}}.}}
In line 3 of Algorithm~\ref{alg:gd}, the function {\em gradient\_calc}
is used to obtain the gradient of the cost function, $\nabla E$, in
terms of each parameter as follows:
\begin{equation}
  \nabla E = \left(\frac{\partial E}{\partial p_0}, \ldots ,\frac{\partial
      E}{\partial p_{n-1}}\right).
\end{equation}

Then, in lines 4-6, the gradient is used to update the parameters
according to $\bm{\eta}$ in a direction that will reduce the cost
function. In line 5, each parameter is changed according to $\partial
E/\partial p_i$ at an update rate of $\bm{\eta}$, which is assumed to be
constant throughout the parameter extraction for the sake of
simplicity. However, the variable step size can be chosen as proposed in
AdaGrad~\cite{JMLR2011_Duchi} or AdaDelta~\cite{arxiv2012_adadelta}.
%;this will be further explained later.

Next, the cost function and its gradient are recalculated based on the
updated model parameters. The gradient calculation and the parameter
update are alternatively repeated until either of the exit conditions in
line 2 is satisfied, i.e., the cost function becomes smaller than the
target value or the iteration limit is reached.

% {\rev{
% It is noted that the parameter extraction is conducted before the
% circuit simulation. Using the model parameter derived by the parameter
% extraction, circuit simulation is performed.}}


\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{Gradient-descent-based parameter optimization}
    \label{alg:gd}
    \begin{algorithmic}[1]
      \Require $\bm{p}=(p_0, \ldots ,p_{n-1})$,
      $\bm{\delta}=(\delta_0, \ldots ,\delta_{n-1})$,
      ${\bm V}=((V_{\rm{gs}_0},
      V_{\rm {ds}_0}), \ldots ,(V_{\rm{gs}_{m-1}},V_{\rm{ds}_{m-1}}))$,
      $\bm{I}^{\rm meas}=(I^{\rm meas}_0, \ldots ,I^{\rm meas}_{m-1})$,
      $E_{\rm target}$, $N_{\rm max}$,
      $\bm{\eta}=(\eta_0, \ldots, \eta_{n-1})$
      \State initialize $N_{\rm iter}=0$
      \Do
      \State $\nabla E, E =$ gradient\_calc($\bm{p}$, $\bm{\delta}$,
      ${\bm V}$, $\bm{I}^{\rm meas}$)
      \ForEach {$p_i \in \bm{p}$}
      \State $p_i = p_i - \eta_i \frac{\partial E}{\partial p_i}$
      \EndFor
      \State $N_{\rm iter}$++
      \doWhile{($N_{\rm iter} < N_{\rm max}$ or $E_{\rm target} < E$) }
      \State Return optimal parameter $\bm{p}$
    \end{algorithmic}
  \end{algorithm}
\end{figure}

\subsection{Numerical Differentiation}\label{sec:nd}

The gradient-based parameter extraction requires the gradient to be
calculated as shown in line 3 of Algorithm~\ref{alg:gd}.  A simple way
to approximate the derivatives is to adopt ND; in this approach, one of
the model parameters, $p_i$, is slightly changed by a small amount,
$\delta_i$, while the other model parameters and inputs are fixed to
evaluate the change in $E$. This two-point gradient approximation is
versatile as it can be applied even when the model equation is not
expressed using closed-form equations.

The ND-based gradient calculation is conducted by the function {\em
gradient\_calc} in Algorithm~\ref{alg:gd} as summarized in
Algorithm~\ref{alg:nd}. The ND approximates the derivative based on the
slope between the two points; thus, the model equation, $f(\cdot)$, must
be evaluated twice (i.e., once with respect to each model parameter,
$I_{\rm sim1}$ and $I_{\rm sim2}$). $E$ and $E_{\rm delta}$ are the
RMSEs for $\bm{p}$ and $\bm{p}'$, respectively. Based on these errors,
the partial derivative of $E$ is calculated with respect to each
parameter as shown in line 14 of Algorithm~\ref{alg:nd}.

\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{ND-based gradient calculation}
    \label{alg:nd}
    \begin{algorithmic}[1]
      \Function{ND}{$\bm{p}$, $\bm{\delta}$, ${\bm V}$, $\bm{I}^{\rm meas}$}
        \State $e=0$, $e_{\rm delta}=0$
          \ForEach {$(V_{\rm{gs}_j},V_{\rm{ds}_j}) \in \bm{V}$}
          \State $I_{\rm sim1} = f(\bm{p},(V_{\rm{gs}_j},V_{\rm{ds}_j}))$
          \State $e=e+(I^{\rm meas}_j - I_{\rm sim1})^2$
          \ForEach {$p_i \in \bm{p}$}
          \State $\bm{p'} = \bm{p}$
          \State Substitute $p'_i = p_i + \delta_i$ for $i$-th element of $\bm{p'}$
            \State $I_{\rm sim2} = f(\bm{p'},(V_{\rm{gs}_j},V_{\rm{ds}_j}))$
            \State $e_{\rm delta}=e_{\rm delta}+(I^{\rm meas}_j - I_{\rm sim2})^2$
          \EndFor
          \State $E= \sqrt{\frac{e}{m}}$
          \State $E_{\rm delta}= \sqrt{\frac{e_{\rm delta}}{m}}$
          \State $\frac{\partial E}{\partial p_i} = \frac{E_{\rm delta}-E}{\delta_i}$
        \EndFor
        \State Return $\nabla E, E$
      \EndFunction
    \end{algorithmic}
  \end{algorithm}
\end{figure}

{\sntn{
ND in the context of parameter extraction is computationally intensive
as it involves the calculation of the cost function and gradient with
respect to the model parameters, and hence, the evaluation of the
model equation for all combinations of bias voltages and
parameters. In the ND-based method, $f(\cdot)$ is evaluated
$(1+n)mN_{\rm iter}$ times, where $N_{\rm iter}$ is the iteration
count. The calculation time increases linearly as $n$
increases. Hence, the time required to evaluate the partial derivative
will increase for complex models {\sato{having larger number of}} parameters. Moreover,
in the situations where any of the model parameters are involved in
different model equations, the computation becomes more complex as the
parameter extraction has to take all the model equations into account.
For example, oxide thickness is involved in both current and
capacitance equations in typical MOSFET models.  The two model
equations should be evaluated simultaneously during the extraction
such that the consistent
%model parameters
{\sato{parameter values}} for these equations are
obtained.  In the optimization, {\em gradient\_calc} is performed with
respect to each model equation. Thus, the total calculation complexity
is written as the sum of $(1+n)mN_{\rm iter}$ in each model
equation. The proposed method adopts AD to eliminate the iteration
over $n$.}}

% Then, the partial derivatives of the
% {\sato{common}} parameters in multiple characteristics are summed up.}}←
% この説明では、どう計算されるかがわかりにくい気がします。二つのグラフのBP
% での枝がマージされるようなかんたんな例が書けるとよいのですが。というか、
% これは次の章に書くべきでは?
% {\mmm{
%  Thus total calculation
% complexity is written as the sum of $(1+n)mN_{\rm iter}$ in each model
% equation.   }}


% the parameter
% extraction time is reduced in each model equation. Than is, if the model
% equations $f_1(\cdot)$ and $f_2(\cdot)$ have $n_1$ and $n_2$ parameters,
% respectively, the calculation complexity


% {\sato{このパラグラフも、もっとあっさり書いて良い気がします。}}
% {\mmm{ Here, we consider two {\sato{model equations}} $f_1(\cdot)$ and
% $f_2(\cdot)$ whose number of parameters are $n_1$ and $n_2$, and
% measured data points are $m_1$ and $m_2$, respectively.
% %As with the above mention,
% {\sato{The}} calculation complexities are written as $(1 + n_1)
% m_1N_{\rm iter}$ and $(1+n_2) m_2N_{\rm iter}$, respectively. Obviously,
% the calculation time increases linearly as $n$ ($n_1$ and $n_2$)
% increases. Thus, the time required to evaluate the partial derivative
% will increase for more complex models with more parameters. The proposed
% method adopts AD to eliminate the iteration over $n$.}}


==> tex/exp.tex <==
\section{Experiments}\label{sec:exp}

To quantitatively evaluate the effectiveness of the proposed method, the
model parameters for two different MOSFET models were extracted using AD-
and ND-based parameter extraction. A commercially available silicon carbide
(SiC) power MOSFET~\cite{sct2450ke} was used for these measurements.
The experiments were conducted using a Linux PC with an Intel Xeon W5590
3.33\,GHz central processing unit (CPU) using a single thread. The
extraction was implemented using the Python programming language.

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.38\linewidth]{./equiv.pdf}
  \caption{Equivalent circuit of SiC power MOSFET.}
  \label{fig:equiv}
\end{figure}

\subsection{MOSFET Models}\label{sec:model}

The two MOSFET models used in this section are an $N$-th-power-law
model~\cite{TED1991_sakurai} and a surface-potential-based
model~\cite{TPEL2018_Shintani}.  The equivalent circuit of SiC power
MOSFET is shown in Fig.~\ref{fig:equiv}.  The MOSFET model
characterizes the current characteristics $I_{\rm sim}$ and three
terminal capacitances: gate-source capacitance $C_{\rm gs}$,
drain-source capacitance $C_{\rm ds}$, and gate-drain capacitance
$C_{\rm gd}$.  The parameter extraction for the $N$-the-power-law
model uses $I_{\rm sim}$ only, while that for the
surface-potential-based model uses $I_{\rm sim}$, $\cds$, and $\cgd$
in this experiment. Note that $\cgs$
%is removed from the parameter extraction target because it is a trivial
%task as $\cgs$
is modeled as constant as in~\cite{TPEL2018_Shintani}.

%They are briefly described below.

\subsubsection{$N$-th-Power-Law Model}

In this model, the drain current is calculated based on the threshold
voltage, $\prmt{VTH}$, of the MOSFET\@. The saturation voltage,
$V_\mathrm{ds,sat}$, and saturation current, $I_\mathrm{d,sat}$, are
defined as
\begin{align}
  V_\mathrm{ds,sat}&=\prmt{J}\left(V_\mathrm{gs}-\prmt{VTH}\right)^{\prmt{M}}
                     \,\,\,\,\,\textrm{and} \\
  I_\mathrm{d,sat}&=\prmt{K}\left(V_\mathrm{gs}-\prmt{VTH}\right)^{\prmt{N}},
\end{align}
where $\prmt{J}$ and $\prmt{M}$ are the fitting parameters used to
calculate the current in the linear region and $\prmt{K}$ and $\prmt{N}$
are other fitting parameters that are used for the saturation
region. $V_\mathrm{ds,mod}$ replaces $V_\mathrm{ds}$ to represent a
smooth transition between the linear and saturation
regions~\cite{TPEL2018_Shintani}:
\begin{align}
  V_\mathrm{ds,mod} = \frac{V_\mathrm{ds}}{\left[1+\left(\frac{V\mathrm{ds}}
  {V_\mathrm{ds,sat}}\right)^{\prmt{DELTA}}
  \right]^{\frac{1}{\prmt{DELTA}}}},
  \label{eq:delta}
\end{align}
where $\prmt{DELTA}$ controls the smoothness of the transition between
$V_\mathrm{ds,mod}$ and $V_\mathrm{ds,sat}$. The drain current,
$I_\mathrm{sim}$, is calculated based on the channel length modulation
and mobility degradation~\cite{TED2006_Miura,TED2006_Gildenblat} as
follows:
\begin{align}
  I_\mathrm{sim}=&I_\mathrm{d,sat}\left(2-\dfrac{V_\mathrm{ds,mod}}{V_\mathrm{ds,sat}}\right)
   \dfrac{V_\mathrm{ds,mod}}{V_\mathrm{ds,sat}}\times\nonumber\\
   &(1+\prmt{LAMBDA} \cdot V_\mathrm{ds})\,\left[1+\prmt{THETA}\,(V_\mathrm{gs}-\prmt{VTH})\right].
\end{align}
The model parameters of the $N$-th-power-law model are listed in
Table~\ref{tab:sakurai_parameters}.

\begin{table}[t]
  \centering
  \caption{Model parameters of the $N$-th-power-law model~\cite{TED1991_sakurai}}
    \label{tab:sakurai_parameters}
    \begin{tabular}{l|l}\hline
      Parameter & Description \\ \hline
      {\bf VTH} & Threshold voltage [V]  \\
      {\bf K} & Fitting parameter for the linear region [-]  \\
      {\bf M} & Fitting parameter for the linear region [-]\\ 
      {\bf J} & Fitting parameter for the saturation region [-]  \\
      {\bf N} & Fitting parameter for the saturation region [-]  \\
      {\bf LAMBDA} & Channel length modulation [1/V]  \\
      {\bf THETA} & Mobility degradation [1/V]  \\
      \prmt{DELTA}& Smoothing parameter for gradual transition\\
                & between the linear and saturation regions [-]\\ \hline
      \end{tabular}
\end{table}

\subsubsection{Surface-Potential-Based Model}

\begin{table}[!t]
  \centering
  \caption{Model parameters of the current equation in the surface-potential-based model~\cite{TPEL2018_Shintani}}
    \label{tab:sp_parameters}
    \begin{tabular}{l|l}\hline
      Model parameter & Description \\ \hline
      \prmt{TOX} &Oxide thickness [m]\\
      \prmt{VFBC}&Flat-band voltage of the channel region [V]\\
      \prmt{NA}& Acceptor concentration [$\rm cm^{-3}$]\\
      \prmt{SCALE}& Current gain factor [$\rm cm^2/V$]\\
      \prmt{RD}& Parasitic resistance at the drain side [$\Omega$]\\
      \prmt{LAMBDA}& Channel length modulation [1/V]\\
      \prmt{THETA}& Channel mobility degradation [1/V]\\
      \prmt{DELTA}& Smoothing parameter for gradual transition\\
                & between the linear and saturation regions [-]\\
      \hline
    \end{tabular}
\end{table}

\begin{table}[!t]
  \centering
  \caption{Model parameters of the capacitance equation in the surface-potential-based model~\cite{TPEL2018_Shintani}}
  \label{tab:symbol_cv}
  \begin{tabular}{l|l}\hline
    Model parameter & Description \\ \hline
    \prmt{ADS}& Drain-source overlap area [$\rm cm^2$]\\
    \prmt{ND}&Donor concentration [$\rm cm^{-3}$]\\
    \prmt{VBI}& Built-in potential of PN junction [V]\\
    \prmt{COXD}& Gate-drain oxide capacitance [F]\\
    \prmt{AGD}& Gate-drain overlap area [$\rm cm^2$]\\
    \prmt{VFBD}& Gate-drain flat-band voltage [V]\\ \hline
  \end{tabular}
\end{table}

\begin{table}[!t]
  \centering
  \caption{Physical constants}
  \label{tab:physical_parameters}
  \begin{tabular}{l|l|r}\hline
    Parameter & Description & Value \\ \hline
    $k$ & Boltzmann's constant [$\rm J/K$] & $1.38 \times 10^{-23}$\\
    $q$ & Elementary charge [C] &$1.60\times 10^{-19}$\\
    $T$& Absolute temperature [K] & 298\\
    $\phi_{\rm t}$& Thermal voltage ($kT/q$) [V] & 0.026\\
    $\varepsilon_{\rm SiC}$ &Permittivity of SiC [F/m] & $9.7\times 8.85 \times 10^{-12}$\\
    $\varepsilon_\mathrm{ox}$ & Permittivity of gate oxide [F/m]& $3.9\times8.85\times10^{-12}$\\
    $n_i$ & Intrinsic carrier concentration & $4.82\times10^{15}$\\ 
     & of SiC [$\rm cm^{-3}$] & \\
    \hline
  \end{tabular}
\end{table}
The proposed parameter extraction is also performed on the
surface-potential-based model, which was developed to simulate the
behavior of a SiC power MOSFET~\cite{TPEL2018_Shintani}. The model
parameters of the current and capacitance model equations are listed
in Tables~\ref{tab:sp_parameters} and~\ref{tab:symbol_cv},
respectively.  The physical constants for these models are summarized
in Table~\ref{tab:physical_parameters}.

According to the current model in~\cite{TPEL2018_Shintani}, the surface
potentials, $\phi_\mathrm{sS}$, and $\phi_\mathrm{sD}$ are first
calculated for the source and drain ends of the channel as functions of
$V_{\rm gs}$ and $V_{\rm ds}$. The inverted charge of the channel is
determined as a function of the surface potential. Then, the
intermediate value $I_{\rm DD}$ in~(\ref{eq:equation}) is computed based
on $\phi_{\rm sS}$ and $\phi_{\rm sD}$ as follows:
\begin{align}
  I_{\rm DD}&=C_{\rm ox}{  (V_{\rm gs} -
        {\bf VFBC} + \phi_{\rm t})(\phi_{\rm sD} - \phi_{\rm sS})} \nonumber \\
  &- \cfrac{1}{2}\, C_{\rm ox}
    (\phi_{\rm sD}^2 - \phi_{\rm sS}^2) \nonumber \\
  &-\cfrac{2}{3}\, \phi_{\rm t} \gamma \left\{\left(\phi_{\rm sD}/\phi_{\rm t}
        - 1\right)^{\frac{3}{2}} - (\phi_{\rm sS}/\phi_{\rm t} -
    1)^{\frac{3}{2}}
    \right\} \nonumber \\
  &+\phi_{\rm t} \gamma
      \left\{\left(\phi_{\rm sD}/\phi_{\rm t} - 1\right)^{\frac{1}{2}} -
    (\phi_{\rm
    sS}/\phi_{\rm
    t} - 1 )^{\frac{1}{2}}\right\},
    \label{eq:idd}
\end{align}
where
\begin{align}
\gamma&=\sqrt{2\varepsilon_{\rm SiC}kT\cdot {\bf NA}}.
\end{align}
Here, $k$ and $T$ are the Boltzmann's constant and the absolute temperature,
respectively. $\varepsilon_\mathrm{SiC}$ is the permittivity of SiC,
$\phi_{\rm t}$ is the thermal voltage, and $C_{\rm ox}$ is gate oxide
capacitance per unit area. Further,
$C_{\rm ox}=\varepsilon_{\rm ox}/{\bf TOX}$, where $\varepsilon_{\rm ox}$
and {\bf TOX} are the permittivity and thickness, respectively, of the gate
oxide. {\bf VFBC} and {\bf NA} are the flat-band voltage and the acceptor
concentration, respectively. The channel current model also includes a
smooth transition between the linear and saturation regions according to the
model parameter {\bf DELTA}, which is defined by a similar equation to that
in the $N$-th-power-law model. Finally, substituting $I_{\rm DD}$
in~(\ref{eq:idd}), the simulated drain current, $I_{\rm sim}$, is
derived. The drain current in the structure also depends on the parasitic
resistance {\bf RD}~\cite{TED2013_Mattausch} which reduces internal drain
voltage of the MOSFET.

In the surface-potential-based model, the calculation of $\phi_{\rm sS}$
and $\phi_{\rm sD}$ involves solving a non-linear
equation~\cite{Baliga_book}, whose solution cannot be explicitly
expressed. Typically, the surface potentials have to be obtained using
iterative methods~\cite{TED2006_Miura,TED2013_Mattausch} such as the
Newton-Raphson method. Though the computational graph
may also be constructed for the model equations
containing
%a limited number of
iterations,
%the computational graph becomes large.
%To avoid this situation, in this experiment,
we adopt the following closed-form expression for the surface potential
$\phi_{\rm s}$~\cite{SSE2001_Chen} for simplifying the
calculation graph:
\begin{align}
  (V_{\rm gs}-\prmt{VFBC}-\phi_{\rm s})^2= \gamma^2 \phi_{\rm t}
  [(\exp(-\frac{\phi_{\rm s}}{\phi_{\rm t}})+\frac{\phi_{\rm s}}{\phi_{\rm t}}-1) +
  \nonumber \\
  \exp(-(2\phi_{\rm F} + \phi_{\rm t})/\phi_t)(\exp(\frac{\phi_{\rm s}}{\phi_{\rm
  t}}) - \frac{\phi_{\rm s}}{\phi_{\rm t}} -1)].
  \label{eq:spe}
\end{align}
$\phi_{\rm sS}$ and $\phi_{\rm sD}$ are derived by solving~(\ref{eq:spe})
with respect to~$\phi_{\rm s}$ at $\phi_{\rm F}=0$ and
$\phi_{\rm F}=V_{\rm ds}$, respectively. Thus, the model equations of the
surface-potential-based model can be entirely represented by a computational
graph.

The capacitance characteristics, $\cds$ and $\cgd$, are expressed in the
surface-potential-based model as follows:
\begin{align}
  C_{\rm ds} &= {\bf ADS}\cdot
               \sqrt{\frac{q \cdot \varepsilon_{\rm SiC}\cdot {\bf ND}}
               {2({\bf VBI} + V_{\rm ds}) }}\,\,\,\,\,\,{\rm and}
               \label{eq:cds} \\
  C_{\rm gd} &= {\bf  COXD} \parallel C_{\rm dep}.
               \label{eq:cgd}
\end{align}
$\cds$ is a bias-dependent junction capacitance between drain and
source, which is calculated on the basis of the capacitance model of
the PN junction as shown in~(\ref{eq:cds}).  $\cgd$ is modeled as a
series connection of the constant gate oxide capacitance ${\bf COXD}$
and the bias-dependent depletion-layer MOS capacitance $C_{\rm dep}$.
Here, $C_{\rm dep}$ is a MOS capacitance represented as a function of
the surface potential $\phi_{\rm gd}$ of the channel formed on the
drain region under the junction field effect transistor (JFET)
region. It can be written as shown in~(\ref{eq:cdep}), where
$\phi_{\rm gd}$ is computed in a similar way to the calculation of
$\phi_{\rm s}$ using \eqref{eq:spe} with ($V_{\rm gd}$, $V_{\rm ds}$,
${\bf ND}$, ${\bf VFBD}$).
% $C_{\rm dep}$ is represented as a function of the surface potential
% $\phi_{\rm gd}$ of the channel formed on the drain region under the
% junction field effect transistor (JFET) region as shown
% in~(\ref{eq:cdep}) {\sato{よくわからない、あと下にも同様の説明がある??}}.

% by replacing ($V_{\rm gs}$, $\phi_{\rm f}$, ${\bf NA}$, $V_{\rm fbc}'$)
% with ($V_{\rm gd}$, $V_{\rm ds}$, ${\bf ND}$, ${\bf VFBD}$), respectively

\begin{figure*}[!t]
  \begin{equation}
      C_{\rm dep} = {\bf AGD}\cdot\sqrt{2q\varepsilon_{\rm SiC}\cdot{\bf
          ND}}
      \, \cfrac{1 - e^{-\phi_{\rm gd}/\phi_{\rm t}} + e^{-(2\phi_{\rm F}+
          V_{\rm ds})/
          \phi_{\rm t}} (e^{\phi_{\rm gd}/\phi_{\rm t}} - 1) }
      {2\sqrt{\phi_{\rm t}e^{-\phi_{\rm gd}/\phi_{\rm t}} + \phi_{\rm gd}
          - \phi_{\rm t} + e^{-(2\phi_{\rm F}+V_{\rm ds})/\phi_{\rm t}}
          (\phi_{\rm t}e^{\phi_{\rm gd}/\phi_{\rm t}} - \phi_{\rm gd} - \phi_{\rm t}) }}
      \label{eq:cdep}
    \end{equation}
\end{figure*}


\subsubsection{Initial Parameter Determination}\label{sec:initial}

\begin{figure}[!t]
  \begin{minipage}{0.48\hsize}
    \begin{center}
      \includegraphics[width=.9\columnwidth]{./lambda_rd.pdf}
    \end{center}
    \caption{Extraction of {\bf LAMBDA} and {\bf RD}.}
    \label{fig:ext_idvd}
  \end{minipage}
  \hspace{2mm}
  \begin{minipage}{0.48\hsize}
    \begin{center}
      \includegraphics[width=.98\columnwidth]{./k_theta.pdf}
    \end{center}
    \caption{Extraction of {\bf K} and {\bf THETA}.}
    \label{fig:ext_idvg}
  \end{minipage}
  \hspace{2mm}
  \begin{minipage}{0.48\hsize}
    \vspace{2mm}
    \begin{center}
      \includegraphics[width=.98\columnwidth]{./cgs.pdf}
    \end{center}
    \caption{Extraction of {\bf VFBC}.}
    \label{fig:ext_vfbc}
  \end{minipage}
  \hspace{2mm}
  \begin{minipage}{0.48\hsize}
    \begin{center}
      \includegraphics[width=.9\columnwidth]{./coxd_vfbd.pdf}
    \end{center}
    \caption{Extraction of {\bf COXD} and {\bf VFBD}.}
    \label{fig:coxd_vfbd}
  \end{minipage}
\end{figure}

{\sntn{The initial parameter determination is one of the important
steps in the model development because the model parameters are
{\sato{repeatedly}} updated
to minimize the discrepancy with the measured device characteristics,
starting {\sato{from the}} initial values.
%in the parameter extraction
%Depending on the
{\sato{When the choice of the}} initial parameters {\sato{is
inappropriate}}, the model parameters may be determined as a local
optimum solution that {\sato{can be}} far from the {\sato{ground
truth}}. The standardized compact models provide the initial parameter
determination as well as the model
descriptions~\cite{BSIM48,HiSIM-HV}.}}  In the experiment, we apply an
initial parameter determination for the surface-potential-based model
proposed in~\cite{WIPDA2019-Shintani}.  In this work, we assume {\bf
TOX} is 50\,nm. The default value of {\bf DELTA}, which is introduced to
model the gradual transition between the linear and saturation regions,
is set to 0.8~\cite{HiSIM-HV}.

The slope of the $I_{\rm d}$-$V_{\rm ds}$ curve in the
saturation region is represented by {\bf LAMBDA}, while that
at $V_{\rm ds} \simeq 0$\,V of a high $V_{\rm gs}$ shows {\bf RD} as
shown in Fig.~\ref{fig:ext_idvd}.  {\bf K} and {\bf THETA}
are extracted from the $I_{\rm d}$-$V_{\rm gs}$ curve as shown in
Fig.~\ref{fig:ext_idvg}.  {\bf K} is approximated by the slope of
saturation-region current, and
%the $\sqrt{I_{\rm d}}$-$V_{\rm gs}$ in the saturate region.
{\bf THETA} is extracted from
%the $I_{\rm d}$-$V_{\rm gs}$ at
the linear region current.
%{\bf ALPHA} is extracted as the voltage where the slope starts to decrease.
{\bf VFBC} is the flat-band voltage of the MOS interface at the
channel region.  Beyond that voltage, the depletion capacitance
becomes apparent in the MOS capacitance characteristics.  Hence, {\bf
  VFBC} can be estimated from the gate-source capacitance $C_{\rm gs}$
against $V_{\rm gs}$ at which $C_{\rm gs}$ starts to bend, as shown in
Fig.~\ref{fig:ext_vfbc}.


As a good estimate, we approximate $C_{\rm dep}$ to a PN
junction capacitance that depends on drain-source voltage
$\vgd$~\cite{EPE2011_Phankong}:
\begin{eqnarray}
  C_{\rm dep} = {\bf AGD}
  \sqrt{\frac{q \cdot \varepsilon_{\rm SiC}\cdot {\bf ND}}{2({\bf VFBD}-\vgd)}}.
  \label{eq:approximated_cgd}
\end{eqnarray}
As shown in Fig.~\ref{fig:coxd_vfbd}, {\bf VFBD} and {\bf COXD} are
obtained as the capacitance in the accumulation mode. {\bf AGD} is estimated
as $\frac{\bf TOX}{\varepsilon_{\rm SiC}{\bf COXD}}$. Then, by substituting
{\bf VFBD}, {\bf COXD}, and {\bf AGD} to~(\ref{eq:approximated_cgd}), {\bf ND}
can be calculated. Finally, {\bf NA} is obtained from
\begin{equation}
 {\bf VBI} = \frac{kt}{q}\ln \left(\frac{{\bf NA} \cdot {\bf ND}}{n_i^2}
 \right),
 \label{eq:vbi}
\end{equation}
where $n_i$ is the intrinsic carrier concentration. {\bf VBI} is derived
as the forward voltage where the body-diode current starts to flow.
{\bf ADS} is calculated by substituting {\bf VBI} and {\bf ND} to (\ref{eq:cds}).

\subsubsection{Computational Graph}
\label{sec:graph}

{\mchr{The computational graphs of the two models were constructed based
on the respective model equations.  {\sato{Graph manipulations are
implemented}} using a Python package, NetworkX~\cite{SCIPY2008_Hagberg}.
As shown in Table~\ref{tab:generation_time}, {\sato{the execution time}}
was {\sato{much}} less than 0.1\,second {\sato{on the single thread PC for
both models}}.  Table~\ref{tab:graph_size} summarizes the sizes of the
two computational graphs from the input parameters to $I_{\rm sim}$ for
a particular bias voltage.  The subgraph for calculating $I_{\rm sim}$
is reused for different bias voltages. The {\sato{graph size of the}}
surface-potential-based model
is approximately ten times larger than {\sato{that of}}
the $N$-th-power-law model. Thus,
only the computational graph of the $N$-th-power-law model is presented
in Fig.~\ref{fig:graph_n-th-power}.
%due to the space limitation.
Through defining the forward and backward functions of each node and
incorporating the computational network into Algorihgm~\ref{alg:ad}, the
AD-based parameter extraction is carried out according to
Algorithm~\ref{alg:gd}.}}


\begin{figure}[!t]
  \centering
  \includegraphics[width=1.0\linewidth]{./level2.pdf}
  \caption{Computational graph of the $N$-th-power-law model for a particular bias voltage.}
  \label{fig:graph_n-th-power}
\end{figure}


\begin{table}[!t]
%  \setcounter{figure}
  \caption{Graph generation time}\label{tab:generation_time}
  \centering
  \begin{tabular}{l|l||r}
    \hline
    \multicolumn{2}{l||}{Model}    & Time {[}s{]} \\ \hline
    \multicolumn{2}{l||}{$N$-th-power-law model} & 0.0384         \\ \hline
    \multirow{3}{*}{Surface-potential-based model}  & $I_{\rm sim}$ & 0.0571 \\ \cline{2-3}
                                   & $\cds$     & 0.0039        \\ \cline{2-3}
                                   & $\cgd$     & 0.0288         \\ \hline
  \end{tabular}
\end{table}

\begin{table}[!t]
  \caption{Size of the computational graphs}\label{tab:graph_size}
  \centering
  \begin{tabular}{l|l||r|r}
    \hline
    \multicolumn{2}{l||}{Model}    & No. of Edges & No. of Vertices \\ \hline
    \multicolumn{2}{l||}{$N$-th-power-law model} &  39 & 48 \\ \hline
    \multirow{3}{*}{Surface-potential-based model} & $I_{\rm sim}$ & 384 & 540 \\ \cline{2-4}
                                   & $\cds$ & 20 & 20 \\ \cline{2-4}
                                   & $\cgd$ & 318 & 228 \\ \hline
  \end{tabular}
\end{table}


% \begin{table}[t]
%   \caption{Size of the computational graphs}\label{tab:graph_size}
%   \centering
%     \begin{tabular}{l|r|r} \hline
%       & Number & Number \\
%       & of edges & of vertices \\\hline
%       $N$-th-power-law model~\cite{TED1991_sakurai} & 39 & 48 \\ \hline
%       Surface-potential-based model~\cite{TPEL2018_Shintani} & &\\ \hline
%       Current model & 384 & 540 \\
%       $C_{\rm ds}$ model & 384 & 540 \\
%       $C_{\rm gd}$ model & 384 & 540 \\ \hline
%     \end{tabular}
% \end{table}


\subsection{Simulation Setup}
I-V curves of the SiC MOSFET~\cite{sct2450ke} were measured at room
temperature using a dedicated curve tracer~\cite{ICMTS2016_Nakamura}
while sweeping $V_{\rm gs}$ from 6\,V to 14\,V with 2\,V steps and
sweeping $V_{\rm ds}$ from 0\,V to 50\,V with 2\,V steps (the total
number of bias voltages tested $m$, were 125). C-V curves were
measured by a commercial curve tracer~\cite{b1505a} at 1\,MHz. The
data points are 300 for both $\cds$ and $\cgd$ measurements.  The
parameter updating process was conducted by using
AdaGrad~\cite{JMLR2011_Duchi}:
\begin{eqnarray}
  h_i &=& h_i + \left(\frac{\partial E}{\partial
          p_i}\right)^2 \qquad {\mathrm{and}}\label{eq:adagrad1} \\
  p_i &=& p_i - \eta_i \frac{1}{\sqrt{h_i}} \frac{\partial E}{\partial p_i}.
  \label{eq:adagrad2}
\end{eqnarray}
The parameter update is performed to decrease the RMSE between the
measured drain current and that obtained through the MOSFET model with
the latest model parameters.  In AdaGrad, the parameter vector,
$\bm{h}=(h_0,...,h_{n-1})$, is introduced. Based on the gradient,
$\eta_i \frac{1}{\sqrt{h_i}}$ is gradually reduced as shown
in~(\ref{eq:adagrad1}) and~(\ref{eq:adagrad2}). Generally, the initial
values of all elements of $\bm{h}$ were set to zero and all elements of
$\bm{\eta}$ were set to 1/100 for the respective parameter values.

\subsection{Results}
\subsubsection{Parameter extraction for current characteristics}\label{sec:c-1}
The parameters extracted by the proposed AD-based approach was
compared with those by the ND-based method using each of the two
MOSFET models. In this experiment, the maximum number of iterations,
$N_{\rm max}$, was set to 1,000 for both the models.  Also, $E_{\rm
  target}$ was set to 0.04\,A and 0.16\,A for each model.  The initial
values are randomly determined for the $N$-th-power-law model, while
those of the surface-potential-model are determined by the initial
parameter determination procedure described in
Section~\ref{sec:initial}. Fig.~\ref{fig:result1} shows the RMSE as
function of the computation time.  The proposed method accelerated the
parameter extraction by 4.03$\times$ and 4.34$\times$ for the
$N$-th-power-law model and the surface-potential-model, respectively.
This improvement in the computation time was close to the theoretical
value of 4.5 ($= (8+1)/2$) for a generalized model with eight
parameters.

\begin{figure}[t!]
  \centering
  \subfigure[$N$-th-power-law model \label{fig:npower}]{
    %\includegraphics[width=0.55\linewidth]{fig/RMSE_thr_model.pdf}}\\
    \includegraphics[width=0.55\linewidth]{./RMSE_thr.pdf}}\\
  \subfigure[Surface-potential-based model\label{fig:sp}]{
    %\includegraphics[width=0.55\linewidth]{fig/Ids_RMSE.pdf}}
    \includegraphics[width=0.55\linewidth]{./RMSE_pot.pdf}}
  \caption{RMSE as a function of the computation time.} \label{fig:result1}
\end{figure}

% \begin{figure}[t!]
%   \centering
%   \subfloat[{\shintani{$N$-th-power-law model}} \label{fig:npower}]{%
%     \includegraphics[width=0.53\columnwidth]{fig/RMSE_thr_model.pdf}
%   }\\
%   \centering
%   \subfloat[{\shintani{Surface-potential-based model}}\label{fig:sp}]{%
%     \includegraphics[width=0.53\columnwidth]{fig/Ids_RMSE.pdf}
%   }
%   \caption{{\shintani{RMSE as a function of the computation time.}}}
%   \label{fig:result1}
% \end{figure}

\begin{figure}[t!]
  \centering
  \subfigure[$N$-th-power-law model \label{fig:sakurai}]{%
    \includegraphics[width=.62\columnwidth]{./thr_model_I-V.pdf}
  }
  \\
  \centering
  \subfigure[Surface-potential-based model \label{fig:iv_sp}]{%
    \includegraphics[width=.65\columnwidth]{./Ids.pdf}
  }
  \caption{Simulated and measured I-V curves.}
  \label{fig:iv}
\end{figure}

The measured and simulated I-V characteristics of the two models are
presented in Fig.~\ref{fig:iv}. The final model parameters extracted using
the AD and ND methods are used to generate the graph. These results show
that both MOSFET models accurately reproduced the I-V characteristics of the
SiC MOSFET\@. The extracted parameter values at $N=N_{\rm max}$ are
summarized in Tables~\ref{tab:sakurai_error} and~\ref{tab:sp_error}. Also,
the initial values are listed in Table~\ref{tab:sp_error} for the
surface-potential-based model. The relative error was smaller than 2\% in
all cases. In addition, it can be seen from Table~\ref{tab:sp_error} that
the initial and the optimized parameters are close with each other,
suggesting that the good initial parameters have been extracted through the
procedure. Hence, it was concluded that the proposed method
accelerates parameter extraction without affecting the accuracy.

\begin{table}[!t]
  \centering
  \caption{Extracted values for the $N$-th-power-law model}
  \label{tab:sakurai_error}
  \begin{tabular}{l||r|r|r} \hline
    &  &  & Relative  \\
    Parameter & AD & ND &  error [\%]  \\ \hline
    {\bf VTH} & 2.600 & 2.600 & 0.116 \\
    {\bf K} & $ 2.691 \times 10^{-3}$& $2.681 \times 10^{-3}$& 0.372 \\
    {\bf N} & 3.284 & 3.286 & 0.061\\
    {\bf LAMBDA} & $2.606 \times 10^{-3}$ & $2.259\times10^{-3}$ & 0.576 \\
    {\bf THETA} & $3.440 \times 10^{-4}$ & $3.464 \times 10^{-4}$ &0.610 \\
    {\bf M} & 1.743 & 1.744 & 0.057 \\
    {\bf J} &0.119 & 0.119 & 0.000 \\
    {\bf DELTA} & 1.269 & 1.267 & 0.158 \\ \hline
  \end{tabular}
\end{table}

\begin{table}[!t]
  \centering
  \caption{Extracted values for the surface-potential-based model}
  \label{tab:sp_error}
  \begin{tabular}{l||r|r|r} \hline
    Parameter&  &  & Relative  \\
    (Initial value) & AD & ND & error [\%]  \\ \hline
    {\bf SCALE} & & &  \\
    (5166360) & 5403054 & 5398779 & 0.079 \\
    {\bf TOX} & && \\
    ($5.0\times 10^{-8}$) & $4.788\times10^{-08}$ & $4.790\times10^{-08}$ & 0.035 \\
    {\bf NA} & &&\\
    ($1.31\times 10^{17}$) & $1.313\times10^{17}$ &$1.313\times10^{17}$& 0.000 \\
    {\bf LAMBDA} & &&\\
    ($8.69\times 10^{-3}$) & $6.110\times10^{-3}$ & $6.086\times10^{-3}$& 0.387 \\
    {\bf VFBC} & &&\\
    ($-4.90$) & $-1.812\times10^{-3}$ &$-1.780\times10^{-3}$ & 1.869  \\
    {\bf THETA} & &&\\
    ($5.91\times10^{-3}$) & $5.912\times10^{-8}$ &$5.941\times10^{-8}$ & 0.492 \\
    {\bf DELTA} & &&\\
    ($0.80$) & 0.6170 & 0.6150 & 0.329 \\
    {\bf RD} & &&\\ 
    ($2.90\times10^{-3}$) & $2.7178\times10^{-3}$ &$2.737\times10^{-3}$ & 0.715  \\ \hline
  \end{tabular}
\end{table}

% \begin{table}[t]
%   \begin{center}
%     \begin{tabular}{c}
%       \begin{minipage}{1.0\hsize}
%         \caption{Extracted values for the $N$-th-power-law model}
%         \label{tab:sakurai_error}
%         \centering
%           \begin{tabular}{l||r|r|r} \hline
%             &  &  & Relative  \\
%             & AD & ND &  error [\%]  \\ \hline
%             {\bf VTH} & 2.600 & 2.600 & 0.116 \\
%             {\bf K} & $ 2.691 \times 10^{-3}$& $2.681 \times 10^{-3}$& 0.372 \\
%             {\bf N} & 3.284 & 3.286 & 0.061\\
%             {\bf LAMBDA} & $2.606 \times 10^{-3}$ & $2.259\times10^{-3}$ & 0.576 \\
%             {\bf THETA} & $3.440 \times 10^{-4}$ & $3.464 \times 10^{-4}$ &0.610 \\
%             {\bf M} & 1.743 & 1.744 & 0.057 \\
%             {\bf J} &0.119 & 0.119 & 0.000 \\
%             {\bf DELTA} & 1.269 & 1.267 & 0.158 \\ \hline
%           \end{tabular}
%       \end{minipage}
%       \\
%       \begin{minipage}{1.0\hsize}
%         \caption{Extracted values for the surface-potential-based model}
%         \label{tab:sp_error}
%         \centering
%         \scalebox{1.0}{
%           \begin{tabular}{l||r|r|r} \hline
%             &  &  & Relative  \\
%             & AD & ND & error [\%]  \\ \hline
%             {\bf SCALE} & 61051 & 60741 & 0.429 \\
%             {\bf TOX} & $6.548\times10^{-08}$ & $6.544\times10^{-08}$ & 0.171 \\
%             {\bf NA} & $1.611\times10^{17}$ &$1.611\times10^{17}$& 0.000 \\
%             {\bf LAMBDA} & $5.258\times10^{-3}$ & $5.203\times10^{-3}$& 0.477 \\
%             {\bf VFBC} & $2.255\times10^{-3}$ &$2.243\times10^{-3}$ & 0.703 \\
%             {\bf THETA} & $9.011\times10^{-8}$ &$8.891\times10^{-8}$ & 0.883 \\
%             {\bf DELTA} & 0.698 & 0.7017 & 0.427 \\
%             {\bf RD} & $6.108\times10^{-5}$ &$6.018\times10^{-5}$ & 1.151 \\ \hline
%           \end{tabular}
%         }
%       \end{minipage}
%     \end{tabular}
%   \end{center}
% \end{table}

\subsubsection{Parameter extraction for multiple
      objectives}\label{sec:multi}
The proposed method can handle model parameters used in different
model equations.  Since {\bf TOX} and {\bf NA} are contained in the
current and capacitance characteristics, $\cds$ and $\cgd$, in the
surface-potential-based model, these parameters have to be consistent
for both characteristics.  In this experiment, the computational
graphs were constructed so that the parameters are simultaneously
optimized for all the model equations.
The cost function is set as the normalized sum of the residuals
to balance the weights of each characteristic.
%The residuals are calculated from the normalized value by maximum
%measurement to cancel the impact of the unit difference.
%Besides, the capacitance are linearized by taking log arithmetic before the
%normalization.
The initial values of the parameters are determined through the
determination procedure.  In this experiment, $E_{\rm target} = 0.02$
was added as the termination condition, in addition to iteration count
$N_{\rm iter} = 1000$.  Since {\bf VBI} can be represented using {\bf
  NA} and {\bf ND} as shown in (\ref{eq:vbi}), the total number of the
model parameters thus is 13 excluding {\bf VBI}.

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.55\linewidth]{./RMSE_sum_2.pdf}
  \caption{RMSE as a function of the computation time for the
        simultaneous parameter extraction.}
  \label{fig:multi_rmse}
\end{figure}

\begin{figure}[t!]
  \centering
  \subfigure[I-V curve]{%
    \includegraphics[width=.65\columnwidth]{./Ids2.pdf}
  }
  \\
  \centering
  \subfigure[C-V curve]{%
    \includegraphics[width=.65\columnwidth]{./sum_Cds_Cgd.pdf}
  }
  \caption{Simulated and measured curves.}
  \label{fig:multi_fit}
\end{figure}

Fig.~\ref{fig:multi_rmse} shows the RMSE as function of computation
time for the simultaneous parameter extraction.  The proposed method
calculates the model parameters 3.50$\times$ faster than the ND-based
parameter extraction. The measured and simulated I-V and C-V
characteristics of the models are presented in
Fig.~\ref{fig:multi_fit}. The graphs are plotted by the final model
parameters extracted using the AD and ND methods. Form the results,
good agreement can be seen among the I-V and C-V characteristics.  The
initial and extracted parameter values when the algorithm exits are
summarized in Table~\ref{tab:sp_multi_error}. The relative error
between the parameters extracted by using the AD and ND methods was
smaller than 3\% in all the parameters. From the result, we confirmed
that the proposed method is applicable for the capacitance
characteristics, and the simultaneous parameter extraction of the
different characteristics.

% {\sato{この後ろの文がよくわかりません}} Supposing $f_1(\cdot)$ and
% $f_2(\cdot)$ are the current and capacitance characteristics,
% respectively, the speedup is thus estimated as 3.0$\times$ from the
% experimental setup and the sum of complexities in each function, and It
% can be concluded that the experimental result is close to the ideal case
% though the small difference is observed due to $E_{\rm target}$.

\begin{table}[!t]
  \centering
          \caption{Extracted values for $I_{\rm sim}$, $\cds$, and $\cgd$ by the
            simultaneous extraction}\label{tab:sp_multi_error}
          \begin{tabular}{l||r|r|r} \hline
            Model parameter & &  & Relative   \\
            (Initial value) & AD & ND & error [\%]  \\ \hline
            {\bf SCALE} &&&\\
            (5166360)  & 5644684 & 5574780 & 1.238\\
            {\bf TOX}  &&& \\
            ($5.00\times10^{-08}$) & $4.933\times10^{-08}$ & $4.947\times10^{-08}$ & 0.286 \\
            {\bf NA} &&& \\
            ($1.31\times10^{17}$) & $1.313\times10^{17}$ & $1.313\times10^{17}$ & 0.000 \\
            {\bf LAMBDA} &&& \\
            ($8.69\times10^{-3}$) & $6.119\times10^{-3}$ & $6.083\times10^{-3}$ & 0.589 \\
            {\bf VFBC} &&&\\
            ($-4.90$) & $-1.943$ & $-1.985$ & 2.168 \\
            {\bf THETA} &&&\\
            ($5.910\times10^{-3}$) & $5.927\times10^{-3}$ & $5.910\times10^{-3}$ & 0.287 \\
            {\bf DELTA} &&&\\
            (0.80) & 0.6073 & 0.6130 & 0.938  \\
            {\bf RD} &&&\\
            ($2.90\times10^{-3}$) & $2.021\times10^{-3}$ & $2.057\times10^{-3}$ & 1.744 \\ \hline
            {\bf ADS} &&&\\
            (0.00776)  & 0.0250 & 0.0250 & 0.000 \\
            {\bf ND}  &&& \\
            ($5.27\times10^{15}$) & $5.266\times10^{15}$ & $5.266\times10^{15}$ & 0.000 \\
            {\bf COXD} &&& \\
            ($4.36\times10^{-10}$) & $4.360\times10^{-10}$ & $4.360\times10^{17}$ & 0.000 \\
            {\bf VFBD} &&& \\
            ($1.00$) & 0.1055 & 0.1055 & 0.000 \\
            {\bf AGD} &&& \\
            ($6.31\times10^{-5}$) & $5.549\times10^{-3}$ & $5.549\times10^{-3}$ & 0.000 \\\hline
          \end{tabular}
\end{table}

\subsubsection{Parameter extraction using LM method}
In addition to the gradient-descent-based method, the proposed method
can be applied to various optimization algorithms that rely on
derivatives.  Here, we show the result of the parameter extraction
derived by incorporating the proposed method with the LM method, which
is adopted in a widely used industrial device modeling
flow~\cite{iccap}.

Fig.~\ref{fig:lm} shows the RMSE reduction in the LM-based parameter
extraction. In this experiment, the model parameters of the
surface-potential-based model are extracted by using the same initial
parameters as those in Sec.~\ref{sec:c-1}.  Owing to the quadratic
convergence property of the LM algorithm~\cite{Computing2005-Fan}, the
number of iterations is reduced to 30 for both the AD- and ND-based
calculations, while the gradient-descent-based method requires more
than six hundred iterations as shown in Fig.~\ref{fig:lm_iter}.
%{\sato{最適化結果は同じだったのか?}}
%in Fig.~\ref{fig:sp}.
% From Fig.~\ref{fig:lm_iter}, it can be seen that the number of iterations
% can be drastically reduced by the LM method algorithm for the AD- and
% ND-based calculations compared to the gradient-descent-based method, which
% requires more than six hundreds iterations in Fig.~\ref{fig:sp}.
%Furthermore,
As expected, close to the ideal 3.89$\times$ acceleration has been
obtained, as shown in Fig.~\ref{fig:lm_time}.
% From Fig.~\ref{fig:lm_time}, we find that the acceleration is slightly lower
% than the theoretical value due to the calculation of the inverse matrix in
% the LM-based optimization, but still, the 3.89$\times$ acceleration is
% obtained.
In addition, the extracted parameters by the AD- and ND-based
calculations, which are shown in Table~\ref{tab:lm_param}, are in
perfect agreement, and quite close to those in
Table~\ref{tab:sp_error}.  From these results, the proposed method can
be successfully applied to other derivative-based optimization
algorithms, and the accelerations according to the number of
parameters can be achieved.

% \begin{figure}[!t]
%   \centering
%   \includegraphics[width=0.55\linewidth]{fig/lm_time.pdf}
%   \caption{{\shintani{RMSE as a function of the computation time for the
%         LM-based parameter extraction.}}}
%   \label{fig:lm}
% \end{figure}

\begin{figure}[t!]
  \centering
  \subfigure[Number of iterations\label{fig:lm_iter}]{
    \includegraphics[width=0.55\linewidth]{./lm_iter.pdf}}\\
  \subfigure[CPU time\label{fig:lm_time}]{
    \includegraphics[width=0.55\linewidth]{./lm_time.pdf}}
  \caption{RMSE reduction in the LM-based parameter extraction.}
  \label{fig:lm}
\end{figure}

\begin{table}[!t]
  \centering
  \caption{Extracted values for the surface-potential-based model in the
    LM-based optimization}
  \label{tab:lm_param}
  \begin{tabular}{l||r|r|r} \hline
    Parameter&  &  & Relative  \\
    (Initial value) & AD & ND & error [\%]  \\ \hline
    {\bf SCALE} & & &  \\
    (5166360) & 516636 & 516636 & 0.000 \\
    {\bf TOX} & && \\
    ($5.0\times 10^{-8}$) & $4.626\times10^{-08}$ & $4.626\times10^{-08}$ & 0.000 \\
    {\bf NA} & &&\\
    ($1.31\times 10^{17}$) & $1.273\times10^{17}$ &$1.273\times10^{17}$& 0.000 \\
    {\bf LAMBDA} & &&\\
    ($8.69\times 10^{-3}$) & $5.312\times10^{-3}$ & $5.313\times10^{-3}$& 0.000 \\
    {\bf VFBC} & &&\\
    ($-4.90$) & $-1.597\times10^{-3}$ &$-1.597\times10^{-3}$ & 0.000  \\
    {\bf THETA} & &&\\
    ($5.91\times10^{-3}$) & $5.910\times10^{-8}$ &$5.910\times10^{-8}$ & 0.000 \\
    {\bf DELTA} & &&\\
    ($0.80$) & 0.614 & 0.614 & 0.000 \\
    {\bf RD} & &&\\ 
    ($2.90\times10^{-3}$) & $2.902\times10^{-3}$ &$2.902\times10^{-3}$ & 0.000  \\ \hline
  \end{tabular}
\end{table}

{\sntn{
\subsection{Manufacturing variability analysis}
Recently, the application of artificial intelligence has been gaining
popularity in the area of power electronics~\cite{TPLE2021_Shuai}. As
an example, a neural network has been applied to model the
{\sato{device}} current characteristics in SPICE
simulators~\cite{TPLE2019_Chiozzi} {\sato{considering the parameter
    fitting as a black-box regression with a neural network.}}
However, {\sato{as opposed to the physics-based modeling,}} neural
networks carry out purely mathematical fitting of the measured device
characteristics to a nonlinear equation, ignoring physical behavior of
the device in interest. In order to fully understand various device
characteristics such as aging-induced threshold voltage
shift~\cite{TED2014_Rescher} and manufacturing process
variation~\cite{APEC2014_Wang,JESTPM2019_Borghese}, which have been
critical issues in the design of power converters using wide-bandgap
semiconductors, the usage of a set of physically meaningful model
parameters is of enormous importance.  {\sato{Although}} the proposed
method incorporates a {\sato{similar}} technique used in neural
networks for model-parameter extraction, our method
%does not eliminate nor alter
{\sato{preserves}} the physical meanings of the model parameters.
}}

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.55\linewidth]{./idvd_var.pdf}
  \caption{{\sntn{Measured I-V characteristics of 35 SiC MOSFETs.}}}
  \label{fig:var}
\end{figure}

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.88\linewidth]{./hist.pdf}
  \caption{{\sntn{Histograms of the extracted model parameters of 35 SiC MOSFETs.}}}
  \label{fig:hist}
\end{figure}

{\sntn{
In order to demonstrate the aforementioned {\sato{advantages}},
we apply the proposed
method to the {\sato{modeling of}} I-V characteristics of 35 SiC MOSFETs, which
%spread as shown 
{\sato{are presented}} in Fig.~\ref{fig:var}.
For instance, in the parallel operation
of SiC MOSFETs in a power module, the
{\sato{characteristics mismatch}}
%variability
causes the current imbalances, resulting in the
significant degradation of the reliability~\cite{APEC2014_Wang}. By
applying the proposed method with the surface-potential-based model,
the distribution of its model parameters can be obtained as shown in
Fig.~\ref{fig:hist}.  We would like to note that the extracted model
parameters {\sato{represent their variation}} 
%can be used for device characterization as bearing the physical meaning
%as opposed to the simple application of
{\sato{while the neural network based method}}~\cite{TPLE2019_Chiozzi}
{\sato{only gives us 35 black box models consisting of slightly
different parameters}}. According to~\cite{JESTPM2019_Borghese}, the
current imbalance can be mitigated by pairing MOSFETs with similar
threshold voltage (${\bf VFBC}$) and/or current gain factor (${\bf
SCALE}$) in parallelly connected SiC MOSFETs. {\sato{Choosing pairs
could be easy with the parameters obtained by the proposed method.}}
Moreover, the distribution of the physically meaningful parameters,
such as {\bf TOX} and {\bf NA}, can {\sato{also}} be used {\sato{by
manufacturers}} to improve manufacturing yields.}}


==> tex/intro.tex <==
\section{Introduction}

%\IEEEPARstart{W}{IDE-BANDGAP}
{\sntn{
Wide-bandgap devices, such as silicon carbide
(SiC) and gallium nitride (GaN) metal oxide semiconductor field-effect
transistors (MOSFETs), are the promising alternatives {\sato{that
replace conventional}} silicon (Si) power
devices~\cite{Baliga_book,Kimoto_book}. Owing to {\sato{the}} excellent
material properties, SiC and GaN MOSFETs can operate at {\sato{higher}}
switching {\sato{frequencies}}
%operations
with lower switching loss
%and higher thermal conductivity.
{\sato{under wide range of ambient temperature.}}  Especially, the high
switching operation greatly contributes to reducing the volume and the
weight of power converters. {\sato{Those are the desirable properties in
the application of}} electric vehicles (EVs), such as on-board charger
(OBC) and in-wheel motor (IWM)~\cite{TIE2917_Liu,ECCE2020_Akatsu}.
%On the other hand, as
As the operating frequency of the power converters increases, design
optimization using circuit simulators based on compact model of
power MOSFETs plays an increasingly important role.}}

%% Therefore, accurate
%% device loss assessment is very important.
%% the key point is accurate
%% prediction of switching losses.
%For metal-oxide-semiconductor field-effect transistors (MOSFETs),

%various types of circuits.

%\cite{TED2006_Miura,SSE2007_He,TED2012_Yao,TED2013_Mattausch,TED2013_Chauhan,TPEL2018_Shintani}
%% {\sntn{
%% The accuracy of the circuit simulation greatly depends on the accuracy
%% of the simulation models, thus research and development of SiC power
%% MOSFET models have been actively conducted.  Among various simulation
%% models that have been proposed for SiC power MOSFETs,
%% surface-potential-based models, which represents the physics of
%% MOSFETs, are gaining popularity.  Excellent agreement between
%% simulated and measured characteristics in both static and dynamic
%% analyses has been
%% demonstrated~\cite{TED2013_Mudholkar,TPEL2016_Tanimoto,TPEL2018_Shintani}.}}

%% the parameter extraction is an important step as well as the
%% development of the simulation model description itself. The
%% determination of the model parameter values is difficult and
%% time-consuming. The determination of the model parameter values is
%% difficult and time-consuming.}}

{\sntn{The formulation of accurate compact models
{\sato{for power MOSETs}},
and the
careful extraction of their parameter sets are crucial for obtaining
reliable results from circuit simulations. Compact power MOSFET
models, which have long been the topic of intensive researches, are
composed of multiple nonlinear functions
%designed to
{\sato{that}} accurately
capture the device physics of the MOSFET.
%Particularly,
{\sato{Recently,}} 
surface-potential-based and charge-based compact
models~\cite{TED2013_Mattausch,TPEL2018_Shintani,TED2019_Agarwal,TED2020_Albrecht}
have been successfully applied to simulate power converters.}}

One of the most widely used parameter-extraction methods is iterative
parameter refinement, which is based on gradient
calculations~\cite{JJAP2004_Li,ICMTS2009_Zhou}.  This approach
involves two processes, gradient calculation and parameter updating,
which are repeated until the characteristics of the model agree with
the measured values, or the iteration limit is reached. In this
context, the gradient is a set of partial derivatives for all model
parameters in the model equation. Then, in the parameter-update phase,
the gradient-descent algorithm is applied to refine the parameters
based on the gradient that indicates the direction in which the
parameters should be adjusted to improve the fitting accuracy.

Although iterative parameter refinement is a very general method and is
applicable to arbitrary model equations, it tends to consume a long time for
all the parameters to converge using this approach. The gradient
calculations require numerical differentiation (ND) with regard to each
parameter, which demands full evaluation of the model equations for all bias
voltages and all model parameters. Therefore, the model evaluation
constitutes most of the time required for parameter optimization. In a
preliminary experiment~\cite{ICMTS2018_Shintani}, even when a very simple
device model equation~\cite{TED1991_sakurai} was used, 99.6\% of the
parameter optimization time was spent on the gradient calculation.

Several techniques are known to derive derivatives: examples include
symbolic differentiation (SD), numerical differentiation (ND), and
automatic differentiation (AD). SD derives derivatives based on the
symbolic rules of basic calculus.  While it provides us with exact
computation, SD tends to require a large amount of memory resource
when the model equation becomes complex. Since ND needs to evaluate
the model equation twice, the calculation time tends to be long
depending on the model scale and the number of model parameters.  AD
is a technique for deriving partial derivatives for the equations
defined in a program. AD can be carried out by the combinations of
four basic arithmetic operations and elementary functions, such as
exponential function, etc., through repeatedly applying the chain
rule.  By using AD, partial derivatives can be automatically obtained
with a reduced calculation cost.

Herein, we propose a method to accelerate the model parameter extraction for
% SPICE compact
power MOSFET models. Expanding upon the idea proposed
in~\cite{ICMTS2018_Shintani}, we implement automatic differentiation
(AD)~\cite{JCAM2000_Bartholomew-Biggs}, which has recently been extensively
applied in machine learning to adjust the weights of convolutional neural
networks during the process of {\it
  backpropagation}~\cite{JMLR2018_Baydin,NATURE2015_LeCun}. The AD technique
enables the contribution of each model parameter to the discrepancy between
the measurement and the model to be calculated individually. This is
achieved by traversing a so-called computational graph merely twice, i.e.,
once in the forward direction and once in the backward direction, regardless
of the number of model parameters. Therefore, the proposed method eliminates
the need for repeated model evaluations during the gradient calculation. The
AD can be directly substituted for the conventional ND so there is no need
to change the existing procedures for updating the parameters in the
gradient-based parameter-extraction method. Herein, we experimentally
demonstrate that this approach reduces the time required for parameter
extraction by 4.34$\times$ than the ND method for a model consisting of eight
parameters; this is close to the theoretical upper limit of 4.5$\times$ time
reduction with this number of parameters.
%{\sato{C 関係のパラ抽と組み合わせるともっと早くなると言わなくてよいか?}}

%% The application of artificial intelligence has been gaining popularity
%% in the area of power electronics~\cite{TPLE2021_Shuai}. As an example,
%% a neural network has been applied to {\sato{model}} the current
%% characteristics in SPICE simulators~\cite{TPLE2019_Chiozzi}. However,
%% neural networks carry out purely mathematical fitting of the measured
%% device characteristics to a nonlinear equation, ignoring physical
%% behavior of the device in interest. In order to fully understand
%% {\sato{various device characteristics}} such as aging-induced
%% threshold voltage shift~\cite{TED2014_Rescher} and manufacturing
%% process variation~\cite{JESTPM2019_Borghese}, which have been critical
%% issues in the design of power converters using wide-bandgap
%% semiconductors, using a set of physically meaningful model parameters
%% is of enormous importance.  The proposed method similarly incorporates
%% a technique used in neural networks for model-parameter extraction,
%% but our method does not eliminate nor alter the physical meanings of
%% the model parameters.

%% {\mmm{The AD has long been known as a powerful tool to automate the
%% calculation of {\sato{partial}} derivatives.  {\sato{Through efficient
%% and effective implementations, AD}} has been {\sato{applied for}}
%% circuit simulation and device
%% modeling~\cite{ISCAS1992_Feldmann,ICCD1992_Melville}.  In {\sato{these
%% literatures, representative use of AD is presented, being operational
%% point}} analysis and sensitivity analysis {\sato{as examples, while the
%% application for model parameter extraction is suggested briefly.}}
%% %there is no demonstration of the parameter extraction.
%% In this manuscript, we revisit the application of AD for the parameter
%% extraction of device parameters.  The effectiveness of the AD-based
%% parameter extraction will be experimentally studied.  We extend the AD-based
%% parameter extraction for optimizing the model parameters that are
%% simultaneously contained in capacitance as well as current model equations.
%% %, whereas the optimization of capacitance characteristics is also skipped in the previous papers.
%% }}

%{\sntn{
%The AD technique is commonly utilized in machine-learning communities
%to learn the weights of artificial neural networks through
%backpropagation~\cite{CORR2015_Baydin,NATURE2015_LeCun}.
%The proposed method thus is higher versatility since incorporating the
%technique used in neural networks into the model parameter extraction
%while maintaining those physical meanings.

%% The main contributions of this work are summarized as follows:
%% \begin{itemize}
%%   \setlength{\itemsep}{-1pt}
%% \item {\bf{AD-based parameter extraction:}} Our method
%%   enables us to accurately model the spatial correlation on the wafer even
%%   for the measurement of RF circuits with the discontinuous changes for any
%%   lots by applying the GP separately to the correct clusters obtained
%%   from the site information.
%% \item {\bf{Active sampling algorithm under multi-site testing environment:}}
%%   We propose an efficient sampling algorithm based on the predictive
%%   variance of the estimation to determine the sample location.
%% \end{itemize}


% {\shintani{The AD has long been known as a method to effectively derive
% partial derivatives in numerical analysis {\sato{これなんのこと?
% jacobian?}}, and is widely used in commercial software in various fields
% thus far {\sato{ここで引用必要}}.  Thus, the AD has {\sato{also}} been used in
% %also
% circuit simulation and parameter optimization for compact
% model~\cite{ISCAS1992_Feldmann,ICCD1992_Melville}.  However, the
% application {\sato{of XXX}} is limited {\sato{to?}} dc analysis in
% circuit simulation and {\sato{to}} current-voltage characteristics in
% model parameter extraction {\sato{引用、current-voltage characteristics
% というのがよくわからない}}.  The biggest advantage of the proposed
% method against the previous works is that the proposed method can
% extract the model parameters for multi-objective functions
% %including
% {\sato{such as?}}
% current and capacitance characteristics simultaneously.
% %As
% {\sato{The}}
% model
% parameters {\sato{that}} are related with {\sato{both}} current and
% capacitance characteristics, such as oxide thickness, the
% %most accountable
% {\sato{consistent}}
% model parameter values
% for them can be obtained by single parameter extraction.
% %Also we would like to note that
% The proposed method can {\sato{also}} be incorporated into LM-based
% parameter extraction with remarkable affinity {\sato{(???)}}, it
% forcuses on accerelating the calculation of partial derivatives
% {\sato{(???)}}.  In experimental results, it is demonstrated that the
% proposed method achieves also 3.9$\times$ accerelation {\sato{理想は何倍?}} in the LM-based
% framework.}}

The remainder of this paper is organized as follows:
Section~\ref{sec:conv} provides the problem formulation of the ND. In
Section~\ref{sec:propose}, the basic concept of AD and the AD-based
parameter-extraction method are described. Then, experiments using two
SPICE models~\cite{TED1991_sakurai,TPEL2018_Shintani} to quantitatively
evaluate the effectiveness of the proposed method are reported in
Section~\ref{sec:exp}. Finally, the paper is concluded in
Section~\ref{sec:conclusion}.


==> tex/propose.tex <==
\section{Parameter extraction based on automatic differentiation}
\label{sec:propose}

The proposed novel method of parameter extraction essentially follows the
same procedure as gradient-based extraction shown in
Algorithm~\ref{alg:gd}. By replacing the most time-consuming step of the
differentiation in ND, AD is expected to significantly reduce the time
required for parameter extraction.

\subsection{Automatic Differentiation}

%% {\shintani{{\sato{Several}} techniques {\sato{are known}} to derive
%% derivatives: {\sato{examples include}} symbolic differentiation, ND, and
%% AD. Symbolic differentiation derives derivatives {\sato{based on the
%% symbolic rules of basic calculus.}}
%% %mathematical processing from an original function.
%% While {\sato{it provides us with}} exact computation, {\sato{symbolic
%% differentiation tends to require a large amount of}} memory resource
%% {\sato{when the model equation becomes complex}}.
%% % and resulting slow.
%% ND has the limitations in {\sato{efficiency}} as discussed in
%% Section~\ref{sec:nd}.  AD is a technique for deriving partial derivatives
%% {\sato{for the}} equations defined in a program.
%% %Even for complex equations, 
%% %takes advantage of the fact that it is composed of 
%% {\sato{AD can be carried out by the}} combinations of {\sato{four basic}} arithmetic operations
%% %such as addition, subtraction, multiplication, and division,
%% and {\sato{elementary}} functions {\sato{such as}} exponential function, etc.,
%% %logarithmic, trigonometric functions. and so on, and is realized by
%% {\sato{through}} repeatedly applying the chain rule.  By using AD,
%% partial derivatives can be automatically obtained with a {\sato{reduced}} 
%% calculation cost.}}

The basic concept of AD\footnote[1]{\mchr{According to the direction of the traverse in the
  computational graph, the AD is classified into two distinct types:
  forward type and reverse type~\cite{JMLR2018_Baydin}. We hereafter
  call the reverse-type AD as AD.}}
 is the decomposition of partial derivatives
using the chain rule. The derivative, ${\rm d}y/{\rm d}x$, of a
composite function, $y = p(q(x)) = p(w)$, is written using the chain
rule as follows:
\begin{equation}
 \frac{{\rm d}y}{{\rm d}x}=\frac{{\rm d}y}{{\rm d}w}\frac{{\rm d}w}{{\rm d}x}.
 \label{eq:example}
\end{equation}
The first and second factors of~(\ref{eq:example}) are individually
calculated because ${\rm d}y/{\rm d}w={\rm d}p(w)/{\rm d}w$ and
${\rm d}w/{\rm d}x={\rm d}q(x)/{\rm d}x$. Then, ${\rm d}y/{\rm d}x$ is
derived as the product of these two factors. In AD, the given expression is
generally represented using a directed acyclic graph
called {\em computational graph}~\cite{NIPS2015_Schulman}.

%% According to the direction of the traverse in the computational graph,
%% the AD is classified into two distinct types: forward type and reverse
%% type~\cite{JMLR2018_Baydin}.  While the forward-type AD traverses the
%% chain rule in forward direction, from input variables to output, the
%% reverse-type AD gives the partial derivatives through reverse
%% traverses.  When the number of the model parameters is larger than
%% that of the output parameters, the reverse-type AD is faster.  In the
%% parameter extraction using RMSE as an error metric, the number of the
%% model parameters is usually much larger than that of the output.
%% Hence, the proposed method adopts the reverse-type AD. We hereafter
%% call the reverse-type AD as AD.

The AD computes the gradient with respect to each parameter as
the contribution to the output.  This is realized by two calculation
modes: forward and backward.  In the forward mode, the given expression
is first decomposed into a set of primitive expressions (i.e., the
simplest functions) such as addition and multiplication functions; in
this mode, the model parameters and input values are propagated to
obtain the value of the output.  Then, in the backward mode, the output
variable to be differentiated is given first and the partial derivative
value concerning each partial expression (e.g., ${\rm d}y/{\rm d}w$ and
${\rm d}w/{\rm d}x$ in the above example in (\ref{eq:example})) is
recursively calculated. In the gradient calculation involved in AD, the
partial derivatives with respect to each of the input parameters are
obtained simultaneously through a traversal of the computational graph
in the forward and backward directions; hence, there is no need to
repeat the model evaluation for each parameter.


% {\shintani{
% According to the direction of the traverse in the computational graph, the
% AD is classified into two distinct types: forward type and reverse
% type. While the forward-type AD specifies that one traverses the chain rule
% from ${\rm d}y/{\rm d}x$ to ${\rm d}y/{\rm d}w$ and
% ${\rm d}w/{\rm d}x$~\cite{AE_book1}, the reverse-type AD has the traversal
% from ${\rm d}y/{\rm d}w$ and ${\rm d}w/{\rm d}x$ to
% ${\rm d}y/{\rm d}x$~\cite{AE_book2}  {\sato{この文の説明がわからない}}. When the number of the model parameters
% is lerger than
% {\sato{that}} of the output parameters, the reverse-type AD is faster.
% %but not vice versa.
% {\sato{In the parameter extraction using RMSE as an error metric,}} 
% the number of the model parameters is {\sato{usually}} much larger
% than that of the {\sato{output.   Hence,}}
% %characteristics in the most compact model,
%the proposed method adopts the reverse-type AD.}}

\subsection{Parameter Extraction}

The AD-based gradient calculation, which is executed by the function
{\em gradient\_calc} in line 3 of Algorithm~\ref{alg:gd}, is outlined
in Algorithm~\ref{alg:ad}. Notably, in contrast to
Algorithm~\ref{alg:nd}, there is no nested loop iterating over all
model parameters.  Instead, the forward propagation and backward
propagation are performed in lines 4 and 5, respectively.  $\nabla E$
is derived by summing the gradient for each bias condition, $\nabla
E_{\rm tmp}$.
%% Instead,
%% the forward propagation and backward propagation are performed in lines
%% 4 and 5, respectively.
The input arguments are also simplified than those in ND.  The input
vector $\bm{\delta}$, which represents the small parameter deviation
used for numerically calculating each gradient, is unnecessary in this
method and thus omitted.
%For the consistency with {\em gradient\_calc} in Algorithm~\ref{alg:gd},
%$\bm{\delta}$ is listed in the input parameters in
%Algorithm~\ref{alg:ad}.

% =======
% there is no nested loop iterating over all model parameters. Instead,
% the forward propagation and backward propagation are performed in lines
% 4 and 5, respectively. The input arguments are also simplified than
% those in ND.  {\mmm{{\sato{In addition}}, when considering several
% model equations {\sato{simultaneously}},
% %, if $\nabla E$ has the partial derivatives of the {\sato{common}}
% %parameters in multiple characteristics, such as oxide thickness for
% %current and capacitance equations,
% after performing {\em gradient\_calc}, they are summed up.  {\sato{II に
% 同じ説明がありわかりにくい...}}}}  {\shintani{Note that the input
% vector, $\bm{\delta}$, which represents small parameter deviation
% used {\sato{for calculating difference quotient}} 
% %to numerically calculate each gradient,
% is unnecessary.  For the purpose of the consistency with
% {\em gradient\_calc} in Algorithm~\ref{alg:gd}, $\bm{\delta}$ is listed
% in the input parameters in Algorithm~\ref{alg:ad}.}}
%{\sato{引数にδを残す必要はないと思いますが、どこかで指摘されていましたっけ?}} }}

\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{AD-based gradient calculation}
    \label{alg:ad}
    \begin{algorithmic}[1]
      \Function{AD}{$\bm{p}$, ${\bm V}$, $\bm{I}^{\rm meas}$}
      \State Initialize $e$ and $\nabla E$ to zero
      \ForEach {$(V_{\rm{gs}_j},V_{\rm{ds}_j}) \in \bm{V}$}
      \State Calculate $I_{\rm sim} = f(\bm{p},(V_{\rm{gs}_j},V_{\rm{ds}_j}))$ and $e=e+(I^{\rm meas}_j - I_{\rm sim})^2$ through forward mode
      \State Calculate $\nabla E_{\rm tmp}$ and $\nabla E = \nabla E + \nabla E_{\rm tmp}$  through backward mode
      \EndFor
      \State $E= \sqrt{\frac{e}{m}}$
      \State Return $\nabla E, E$
      \EndFunction
    \end{algorithmic}
  \end{algorithm}
\end{figure}

The computational complexity of the forward and backward propagation
is roughly equal to that of a single model
evaluation~\cite{OMS1992_Griewank}; therefore, the calculation
complexity becomes $2mN_{\rm iter}$ and is independent of the number
of parameters $n$, unlike that in ND. Specifically, comparing the
loops in Algorithms~\ref{alg:nd} and~\ref{alg:ad}, the gradient
calculation is accelerated by the factor of $(n+1)/2$ in AD as
compared to ND. Therefore, as the number of the model parameters
increases, the acceleration efficiency linearly improves.  In
situations where two model equations $f_1(\cdot)$ and $f_2(\cdot)$ are
considered, those calculation complexity becomes merely the summation
of that of each equation, $2m_1N_{\rm iter} + 2m_2N_{\rm iter}$. In
the gradient calculation, if $\nabla E$ has the partial derivatives of
the common parameters in the two models, they are added up.

% {\mmm{Also, when considering the several model equations, if $\nabla E$ has
%     the partial derivatives of the {\sato{common}} parameters in multiple
%     characteristics, such as oxide thickness for current and capacitance
%     equations, they are summed up.}}

The proposed parameter-extraction method is described using a simple example
model: the drain current equation. The drain current equation is expressed
as $f(\cdot)$ in Algorithm~\ref{alg:ad} and is defined as
follows~\cite{TPEL2018_Shintani}:
\begin{align}
  I_{\rm sim} = \cfrac{1}{1 + \prmt{THETA}\cdot V_{\rm gs}} \, (1 +
  \prmt{LAMBDA}\cdot V_{\rm ds}) \nonumber \\
  \cdot{\prmt{SCALE}}\cdot I_{\rm DD}, \label{eq:equation}
\end{align}
where $I_{\rm sim}$ is the simulated drain current, $I_{\rm DD}$ is an
intermediate value expressed as a function of $V_{\rm gs}$, $V_{\rm ds}$,
and the surface potentials at the metal-oxide-semiconductor (MOS)
interface. The channel current equation includes the channel length
modulation and mobility degradation. $\bf{SCALE}$, $\bf{LAMBDA}$, and
${\bf THETA}$ are model parameters that represent the scaling factor,
channel length modulation, and channel mobility degradation, respectively.

\begin{figure}[!t]
 \centering
 \includegraphics[width=0.52\linewidth]{graph.pdf}
 \caption{Computational graph of~(\ref{eq:equation}) including five
 multiplication operations, two addition operations, and one division
 operation.}
 \label{fig:graph}
\end{figure}

Fig.~\ref{fig:graph} shows a computational graph
representing~(\ref{eq:equation}). The variables located at the leaves of the
graph (i.e., {\bf THETA} and $V_{\rm ds}$) represent the inputs and that on
the bottom (i.e., $I_{\rm sim}$) represent the output. The vertices labeled
as $v_1, \ldots, v_7$ stand for intermediate variables. The nodes represent
the basic mathematical function, with each node defining an input variable,
output variable, internal connection, and functional behavior. The order of
the input edges is defined consistently to handle the operations that is
commutative such as subtraction and division.

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.73\linewidth]{./forward_graph.pdf}
  \caption{Forward propagation mode. In this figure, the graph is
  simplified by showing only one subgraph for the current calculation
  of $v_9$.}
 \label{fig:forward_graph}
\end{figure}

In the AD-based gradient calculation, the forward propagation is conducted
first. The current model equation is evaluated by traversing the
computational graph to calculate the internal variables under a particular
bias voltage condition, $V_{\rm ds}$ and $V_{\rm gs}$, as shown in
Fig.~\ref{fig:forward_graph}. During the forward propagation, the values of
the internal vertices, $v_1, \ldots, v_{12}$ and $I_{\rm sim}$, are stored
for use in the backward propagation that will be conducted later. Note that,
in Fig.~\ref{fig:forward_graph}, the calculation of the RMSE is in the last
part of the graph. In the summation operation used to calculate the RMSE,
the values of $I_{\rm meas}-I_{\rm sim}$ for each of the bias voltages are
required. To simplify the illustration, only the graph for $v_9$ is shown
and the subgraphs for the other bias points are omitted.

\begin{figure}[!t]
 \centering
 \includegraphics[width=0.73\linewidth]{./backward_graph2.pdf}
 \caption{Backward propagation mode.  The directions of arrows are
   reversed as compared to those in Fig.~\ref{fig:forward_graph}.  The
   dashed arrows indicate the path from $E$ to {\bf SCALE}. The
   propagated values on the path in the backward propagation are
   highlighted.}
 \label{fig:backward_graph}
\end{figure}

% The AD technique considers the gradient with respect to each parameter as
% the contribution to the error $E$.  This is done,
In the backward mode, the derivative of the output $E$ is propagated
backwards through the graph to calculate the partial derivative with
respect to each model parameter, as shown in
Fig.~\ref{fig:backward_graph}, in which the path to calculate
$\frac{\partial E}{\partial {\bf{SCALE}}}$ has been highlighted as an
example.  There are eight vertices ($E$, $v_{11}$, $v_{10}$, $v_9$,
$v_8$, $I_{\rm sim}$, $v_7$, and ${\bf{SCALE}}$) on the path.  According
to the chain rule, $\frac{\partial E}{\partial {\bf{SCALE}}}$ is
calculated as follows:
\begin{eqnarray}
 \label{eqchain}
  \frac{\partial E}{\partial {\bf{SCALE}}} =
  \frac{\partial E}{\partial v_{11}} \cdot \frac{\partial v_{11}}{\partial v_{10}}
  \cdot \frac{\partial v_{10}}{\partial v_9} \cdot \frac{\partial v_9}{\partial v_8}
  \nonumber  \\
  \cdot \frac{\partial v_8}{\partial I_{\rm sim}}
  \cdot \frac{\partial I_{\rm sim}}{\partial v_7}
  \cdot \frac{\partial v_7}{\partial {\bf{SCALE}}}.
\end{eqnarray}
The derivative of each edge with respect to the previous edge can be
easily obtained: $\frac{\partial E}{\partial
v_{11}}=\frac{1}{2\sqrt{v_{11}}}$ because $E=\sqrt{v_{11}}$.  Similarly,
$\frac{\partial I_{\rm sim}}{\partial v_7}=I_{\rm DD}$ as $I_{\rm
sim}=v_7\cdot I_{\rm DD}$, and $\frac{\partial v_7}{\partial
{\bf{SCALE}}}=v_4$ as $v_7=v_4 \cdot {\bf{SCALE}}$.  Substituting all
the derivatives in~(\ref{eqchain}) with the partial derivatives of
the edges obtained by traversing the graph, the following equation is
derived:
\begin{equation}
  \frac{\partial E}{\partial {\bf{SCALE}}}= \frac{1}{2\sqrt{v_{11}}} \cdot
  \frac{1}{m} \cdot 2v_8 \cdot I_{\rm DD} \cdot v_4.
  \label{eq:lambda}
\end{equation}
The values of $v_{11}$, $v_8$, and $v_7$ were already stored while
progressing the forward mode.  The partial derivatives are calculated
for all model parameters and the resulting set of partial derivatives is
used as a gradient in the parameter updating phase. The chain rule
provides us with a way to easily and efficiently calculate the gradients
without approximation.
%In order to quickly calculate the gradient, in our implementation, the
%
The edges of the graphs for forward and backward propagations can be
determined by simply consulting the rules as summarized in
Fig~\ref{fig:rules}.

We would like to note that the partial derivative shown
in~(\ref{eq:lambda}) is the value of a single bias condition.  When
there are multiple bias conditions, which is usually the case, the
backward propagation explained above is carried out for all bias
conditions.  That is, at the sum node, the partial difference of all
the paths contributing $E$ is calculated for each bias condition until
the model parameter node is reached.  The partial derivatives of the
model parameters are the summation of the partial derivatives of the
different bias voltages diverged at the sum node.


%
\begin{figure}[!t]
  \centering
  \subfigure[Multiplication ($x \cdot y$)\label{fig:mul}]{
    \includegraphics[width=0.3\linewidth]{./mul.pdf}}
  \hspace{2mm}
  \subfigure[Addition ($x + y$)\label{fig:add}]{
    \includegraphics[width=0.3\linewidth]{./add.pdf}}
  \\
  \subfigure[Division ($x/y$)\label{fig:div}]{
    \includegraphics[width=0.32\linewidth]{./div.pdf}}
  \hspace{2mm}
  \subfigure[Summation ($\sum x_m$)\label{fig:sum}]{
    \includegraphics[width=0.32\linewidth]{./sum.pdf}}
  \\
  \subfigure[Exponential ($\exp(x)$)\label{fig:exp}]{
    \includegraphics[width=0.4\linewidth]{./exp.pdf}}
  \\
  \hspace{2mm}
 \subfigure[Square root ($\sqrt{x}$)\label{fig:sqrt}]{
 \includegraphics[width=0.32\linewidth]{./sqrt.pdf}}
\caption{Representative forward and backward propagation rules.  The solid
  arrow is for forward propagation and the dashed one is for the backward
  propagation.  In this figure, a value of 1 is assumed to be the input in
  the backpropagation.} \label{fig:rules}
\end{figure}

% For example, the sum operation is used in the
%calculation of the RMSE\@. The both modes of the sum operation are
%similarly calculated with the addition operation.}}  Most of the
%operations, including the exponential operation, can also be represented
%using the computational graph.
% {\shintani{As the calculation of the RMSE has a
%     reconvergence structure from the output to input, all the reconverged
%     values are summed up at the reconvergence node, then the summed is
%     propagated to downstream.}}

%Note that
The computational graph must be constructed only once for a
given MOSFET model. The construction can be very quick as described in
the experimental section. Additionally, once the computational graph
is generated, it can be reused as long as the same MOSFET model is
used; therefore, the time needed to construct the computational graph
is virtually negligible. Besides, since building a computational graph
on the basis of model equations, either model equations or source
code, at least, is required as a prerequisite for applying the
proposed parameter extraction.
{\sntn{
Note that the extracted model parameters by {\sato{the}} proposed method bears
physical meaning when physics-based model is used as the
computational graph is {\sato{consistent with the model equations.}} 
%constructed while keeping the model quation.
Thus, the estimated model parameters can be used for device
characterization, such as manufacturing variability analysis.}}

%% Note that the computational graph must be constructed only once for a
%% given MOSFET model. The construction can be very quick as described in
%% the experimental section. Additionally, once the computational graph is
%% generated, it can be reused as long as the same MOSFET model is used;
%% therefore, the time needed to construct the calculation graph is
%% virtually negligible.  {\rev{We also note that the proposed method can
%% be applied to {\sato{the}} models that {\sato{are defined implicitly}}
%% and require iterative calculation {\sato{as long as the upper bound of
%% the number of iterations is known apriori.}}
%% %such as the Newton-Raphson method
%% %if the number of iterations is limited. 
%% For example, when the {\sato{values given by the model converges within 10
%%     times of iteration,}} the calculation graph {\sato{is generated
%%     enrolling the equation involved in the loop}} for 10 times.  The
%% calculation graph can then be traversed as presented.}} {\rev{Besides, since
%% building a computational graph on the basis of model equations, either model
%% equations or source code, at least, is required as a prerequisite for
%% applying the proposed parameter extraction.}}

% {\shintani{
% We also would like note that the AD has some limitations. If the model
% equation has unbounded loop, such as {\it while} statement, and {\it if}
% statement, it is difficult to construct the computational graph for the
% model. In order to safely apply the proposed model, such statements should
% be avoid in the model equation.}}

